A Tight Approximation for Submodular Maximization with Mixed Packing and Covering Constraints

Motivated by applications in machine learning, such as subset selection and data summarization, we consider the problem of maximizing a monotone submodular function subject to mixed packing and covering constraints. We present a tight approximation algorithm that for any constant $\epsilon >0$ achieves a guarantee of $1-\frac{1}{\mathrm{e}}-\epsilon$ while violating only the covering constraints by a multiplicative factor of $1-\epsilon$. Our algorithm is based on a novel enumeration method, which unlike previous known enumeration techniques, can handle both packing and covering constraints. We extend the above main result by additionally handling a matroid independence constraints as well as finding (approximate) pareto set optimal solutions when multiple submodular objectives are present. Finally, we propose a novel and purely combinatorial dynamic programming approach that can be applied to several special cases of the problem yielding not only {\em deterministic} but also considerably faster algorithms. For example, for the well studied special case of only packing constraints (Kulik {\em et. al.} [Math. Oper. Res. `13] and Chekuri {\em et. al.} [FOCS `10]), we are able to present the first deterministic non-trivial approximation algorithm. We believe our new combinatorial approach might be of independent interest.

==> tex/vanilla-greedydp.tex <==
\subsection{Forbidden sets for a single packing and a single covering constraints.}\label{subsec:submodular-one}
In this setting we are able to ensure a $(1-\eps)$-violation of the covering constraints by using the concept of \emph{forbidden sets}.
Intuitively, we exclude the elements of these set from being included to the dynamic programming table in order to be able to complete the table entries to solutions with only small violation.
%By a standard guessing procedure, for some fixed $\eps>0$, we assume that $\bP_\ell \leq \eps\cdot \p$ for all elements $\ell\in\cN$. 

\subsubsection{Algorithm}\label{subsubsec:forbiddenAlgorithm}

\noindent {\bf\em{Guessing:}} Fix some $\eps>0$. By guessing we assume that we know the set $G$ of all, at most $1/\eps$ elements $\ell$ from the optimum solution with $\bP_\ell>\eps$. We can guess $G$ using brute force in $n^{O(1/\eps)}$ time. This allows us to remove all elements with $\bP_\ell \geq \eps$ from the instance. Let $\cN'$ be the rest of the elements. (For consistency reasons, we use bold-face vector notation here also for dimension one.)

\noindent {\bf\em{Forbidden Sets:}} Fix an order of $\cN'$ in which the elements are sorted in a non-increasing order of $\bC_\ell/\bP_\ell$ values, breaking ties arbitrarily. Let $\cN_i$ be the set of the first $i$ elements in this order. For any $\p'\leq \p$, let $F_{\p'}$ be the smallest set $\cN_i$ with $\bP\one_{\cN_i}\geq \p-\p'$. Note that the profit of $F_{\p'}$ is at least the profit of any subset of $\cN'$ with packing value at most $\p-\p'$ and that the packing value of $F_{\p'}$ is no larger than $(1+\eps)\p-\p'$. Also note that for any $0 \leq \p'\leq \p'' \leq \p$, it holds that $F_{\p''} \subseteq F_{\p'}$.

Now we explain the modified Greedy-DP which incorporates the guessing and the forbidden sets ideas. 

\noindent {\bf\em{Greedy-DP algorithm with guessing and forbidden sets:}} Let $G$ be the set of the guessed big elements as described above.
For the base case, we set $T[\bC \one_G, \bP \one_G] = G$ and $T[\bc', \p']=\bot$ for all table entries with $\bc' \neq \bC \one_G$ or $\p' \neq \bP \one_G$.

In order to compute $T[\bc', \p']$, we look at every set of the form $T[\bc'-\bC_\ell,\p'-\bP_\ell] \cup \{\ell\}$, where $\ell\in\cN \setminus (T[\bc'-\bC_\ell,\p'-\bP_\ell] \cup F_{\p'})$, such that $\bc'- \bC_\ell \geq 0$ and $\p'- \bP_\ell \geq 0$. Notice that we forbid elements belonging to $F_{\p'}$ to be included in any table entry of the form $T[\bc', \p']$. Now out of all these sets, we assign the most valuable set to $T[\bc', \p']$. The output of our algorithm is the best of the solutions $T[\bc', \p'] \cup F_{\p'}$, such that $\bc' + \bC \one_{F_{\p'}} \geq \bc$.

The pseudo-code of the algorithm can be found below.


  \begin{algorithm*}[H] \label{alg:GreedyDPForbid}
  \caption{Greedy Dynamic Program with Guessing and Forbidden Sets}
  create a table $T\colon [n]_0\times[n \cdot c_{\max}]_0^c\times[p_{\max}]_0^p\rightarrow 2^{\cN}$ initialized with entries $\bot$\label{algline:init}\\
  $S \gets \varnothing$ \\
  \ForEach{$G \subseteq \cN$, such that $|G| \leq 1/\eps, \bP\one_{G}\leq \p$}{
    $T[\bC\one_{G},\bP\one_{G}]\gets G$\\
    \ForEach{$\bc'\in [n \cdot c_{\max}]_0^c$ and $\p' \in [p_{\max}]_0^p$}{
        \ForEach{$\ell\in\cN \setminus (T[\bc'-\bC_\ell,\p'-\bP_\ell] \cup F_{\p'})$\label{algline:forEachElement}}{
            $\bc''\gets\bc'+\bC_{\ell}$, $\p''\gets\p'+\bP_{\ell}$\\
            $T[\bc'',\p''] \gets \arg\max\{f(T[\bc'',\p'']),f(T[\bc',\p']\cup\{\ell\})\}$\label{algline:greedyExtend}\\
        }
    }
    $\displaystyle S \gets \argmax\{f(S), \max_{\substack{\bc', \p':\\ \bc' + \bC \one_{F_{\p'}} \geq \bc}} \{ f(T[\bc',\p']\cup F_{\p'})\}\}$\\
  }
  Output $S$.
  \end{algorithm*}\sumi{Need to create $F_{\p'}$ array.}

\subsubsection{Analysis}\label{subsubsec:forbiddenAnalysis}

\paragraph{A Warmup}
Before stating our analysis based on a factor-revealing LP, we give first a more direct, ``combinatorial'' proof that the above algorithm is a $0.25$-approximation algorithm. The proof already contains some of the ideas and technical ingredients used in the factor-revealing LP.

We first prove the following simple but crucial observation.
\begin{lemma}
Any table entry $T[\bc', \p']\neq\bot$ with $0\leq \p'\leq \p$ and $0\leq \bc'\leq n\bc_{\max}$ is disjoint from $F_{\p'}$. 
\end{lemma}
\begin{proof}
We prove the claim for all entries $T[\bc', \p']\neq\bot$ by induction on $\p'$. Hence we consider only entries $\bc'\geq \bC \one_G$ and $\p'\geq \bP \one_G$. 

The claim clearly holds for $T[\bC \one_G, \bP \one_G] = G$ since $G$ is disjoint from $\cN'$ and since $F_{\bP \one_G}\subseteq \cN'$.

Note that any table entry $T[\bc', \bP \one_G]$ with $\bc'>\bC \one_G$ is $\bot$ as there are no zero-weight elements in $\cN'$. Now consider an entry $T[\bc', \p']\neq\bot$ with $\p'>\bP \one_G$. Let $s^*$ be the element used by the DP for computing this entry, that is, $T[\bc',\p']= \mathrm{pred}(s^*)\cup\{s^*\}$ where $\mathrm{pred}(s^*)=T[\bc'-\bC_{s^*},\p'-\bP_{s^*}]$. By line~\ref{algline:forEachElement} Algorithm~\ref{alg:GreedyDPForbid}, we have that $s^* \notin F_{\p'}$. By the inductive hypothesis, we have on the other hand that $T[\bc'-\bC_{s^*},\p'-\bP_{s^*}]$ is disjoint from $F_{\p'-\bP_{s^*}}$. The claim now follows for $T[\bc',\p']$ because $F_{\p'}\subseteq F_{\p'-\bP_{s^*}}$.
\end{proof}

Let $O$ be an optimal set solution. Let us consider an arbitrary permutation of $O$, say $\{o^1,o^2,\dots, o^k\}$. Let $O^i = \{o^1, \dots, o^i\}$ be the set of the first $i$ elements in this permutation. We define an ``incremental'' gain function $g\colon O \rightarrow \mathbf{N}$. More precisely, let $g(o^i)=f(O^i) - f(O^{i-1})$ be the incremental gain of any element $o^i \in O$. Note that $f(O)= \sum_{o \in O} g(o)$. Let for any subset $S \subseteq O$, $g(S) = \sum_{o \in S}g(o)$.

\begin{lemma}
\label{lem:subset}
For any subset $S\subseteq O$, we have $f(S) \geq g(S)$.
\end{lemma}
\begin{proof}
Let $s^{i_1},\dots, s^{i_p}$ with $i_1<i_2<\dots<i_p$ be the elements of $S$ in the order as they appear in $O$. Let $S_j$ be the set of the first $j$ elements in $S$, that is, $S^j=S\cap O^{i_j}$ for $j=1,\dots,p$, and let $S^0=\emptyset$. By submodularity of $f$ and $S^{j-1}\subseteq O^{i_j-1}$ we have that 
\begin{displaymath}
f(S) = \sum_{j=1}^p f(S^j)-f(S^{j-1}) \geq \sum_{j=1}^p f(O^{i_j})-f(O^{i_j-1}) = \sum_{j=1}^p g(s^{i_j}) = g(S).
\end{displaymath}
\end{proof}


\begin{lemma}
\label{lem:submodular-one}
There is a $0\leq \p'\leq \p$ and a $\bc'\geq 0$ with $\bc' + \bC\one_{F_{\p'}} \geq \bc$ such that $f(T[\bc', \p']\cup F_{\p'})\geq\frac14 f(O)$.
\end{lemma}

\begin{proof}
For the sake of a contradiction let us assume that there is no such table entry as stated in the lemma.

Let $q_0$ be the number of guessed elements in the guessing phase.
We will show that the following claim holds under the assumption that the lemma is not true.
\begin{claim}
For any $q_0 \leq q \leq k$ there is a $q$-subset $O_q=\{o_1,\dots,o_q\}$ of $O$ with total packing value $\p_q$ and total covering value $\bc_q$ such that $O_q$ is disjoint from $F_{\p_q}$ and $f(T[\bc_q, \p_q])\geq \frac12 g(O_q)$ holds.
\end{claim}

Note that this claim already yields the desired contradiction by considering the case $q=k$. To this end, note that $O_k=O$, that by monotonicity we have $f(T[\bc_k, \p_k]\cup F_{\p_k})\geq f(T[\bc_k, \p_k])\geq\frac12g(O_k)=\frac12 f(O)$, and also $\bc_k+\bC \one_{F_{\p_k}})\geq \bc_k = \bC\one_O \geq \bc$.

We now prove the above claim by induction on $q$. The claim is true for $q=q_0$ since we can set $O_{q_0}$ to the set of guessed elements. Then we have $f(T[\bC \one_{q_0},\bP \one_{q_0}])=f(O_{q_0}) \stackrel{\text{Lem.~\ref{lem:subset}}}\geq g(O_{q_0})$.

For the inductive step assume now that $q \geq q_0+1$ and assume that the claim already holds for $q-1$. To this end, let $O_{q-1}$, $\bc_{q-1}$ and $\p_{q-1}$ be as in this claim. Let $S=T[\bc_{q-1}, \p_{q-1}]$.

We distinguish between two cases. In the first case there is an $\ell_q \in O \setminus (O_{q-1}\cup F_{\p_{q-1}})$ such that $f(S \cup \{ \ell_q \}) - f(S) > \frac12 g(\ell_q)$. Note that $\ell_q \notin S$, since otherwise the left hand side of the inequality will be zero while $g(\ell_q)$ is non-negative, which is a contradiction. Now, let $O_{q} = O_{q - 1} \cup \{\ell_q\}$, $\bc_q = \bc_{q-1} + \bC_{\ell_q}$ and $\p_q=\p_{q-1}+\bP_{\ell_q}$. Note that $\ell_q\notin F_{\p_q}$ since $\ell_q\notin F_{\p_{q-1}}$ and $F_{\p_q}\subseteq F_{\p_{q-1}}$, hence the DP can also add this element $\ell_q$ to the entry $T[\bc_{q-1}, \p_{q-1}]$ to get $T[\bc_q, \p_q]$. Now verify that
\[ f(T[\bc_q, \p_q]) \geq f(S\cup\{\ell_q\}) \geq f(S)+\frac12 g(\ell_q) \geq \frac12 \sum_{\ell_i\in O_{q-1}}g(\ell_i)+\frac12 g(\ell_{q}) = \frac12 \sum_{\ell_i\in O_{q}} g(\ell_i). \]

In the second case, for all $a \in O \setminus (O_{q-1}\cup F_{\p_{q-1}})$, we have $f(S \cup \{ a \}) - f(S) \leq \frac12 g(a)$.  In this case we will arrive at a contradiction to our assumption that the lemma is not true.

For this let us define $S'=S$ and $O'=O_{q-1}$ and look at elements in $(F_{\p_{q-1}} \setminus O') \cap O$. If $\exists b \in (F_{\p_{q-1}} \setminus O') \cap O$, such that $f(S \cup \{b\}) - f(S) > \frac12 g(b)$, then we define $S'=S \cup \{b\}$ and $O'=O' \cup\{b\}$. We know by induction hypothesis that $f(S)\geq \frac12 g(O_{q-1}) = \frac12 g(O')$. These two things together imply that $f(S') \geq \frac12 g(O')$. Now we again check whether there $\exists b \in (F_{\p_{q-1}} \setminus O') \cap O$, such that $f(S' \cup \{b\}) - f(S') > \frac12 g(b)$. If yes, then we define $S'=S \cup \{b\}$ and $O'=O' \cup\{b\}$ and get $f(S') \geq \frac12 g(O')$. We iterate this process until $\forall b \in (F_{\p_{q-1}} \setminus O') \cap O$, $f(S' \cup \{b\}) - f(S') \leq \frac12 g(b)$. Note that $S'$ is a union of $S$ and a few elements from $F_{\p_{q-1}} \cap O$. Hence $S\subseteq S'$ and by submodularity of $f$ we get $f(S' \cup \{ a \}) - f(S') \leq f(S \cup \{ a \}) - f(S)$ for any $a \notin S'$. This in turn implies that for all $a \in O \setminus (O_{q-1}\cup F_{\p_{q-1}})$, we have $f(S' \cup \{ a \}) - f(S') \leq f(S \cup \{ a \}) - f(S) \leq \frac12 g(a)$. Note that $(F_{\p_{q-1}} \setminus O') \cap O$ and $ O \setminus (O_{q-1}\cup F_{\p_{q-1}})$ are disjoint and $((F_{\p_{q-1}} \setminus O') \cap O) \cup(O \setminus (O_{q-1}\cup F_{\p_{q-1}})) = O \setminus O'$. Let $O \setminus O' = \{a_1, a_2, \dots a_m\}$. By submodularity of $f$ we have, $f(S' \cup \{a_1, a_2, \dots a_j\}) - f(S' \cup \{a_1, a_2, \dots a_{j-1}\}) \leq f(S' \cup \{a_j\}) - f(S')\leq \frac12 g(a_j)$ for all $j=1,2, \dots m$. Adding up all these inequalities, we get
\begin{align*}
f(S' \cup (O \setminus O'))-f(S') &= \sum_{j=1}^m [f(S'\cup \{a_1,\dots,a_j\}) \\
& \qquad\qquad -f(S'\cup\{a_1,\dots,a_{j-1}\})]\\
& \leq \frac12\sum_{j=1}^m g(a_j)\\
& = \frac12 g(O \setminus O')\,.
\end{align*}

Rearranging, we get
\begin{align*}
f(S') & \geq f(S' \cup (O \setminus O')) - \frac12 g(O\setminus O')\\
 & \geq f(O \setminus O') - \frac12 g(O \setminus O')\\
 & \stackrel{\text{Lem.~\ref{lem:subset}}}{\geq} \frac12 g(O \setminus O')\,.
\end{align*}

Adding this inequality to the final inequality which we get after our iterative process, i.e. $f(S') \geq \frac12 g(O')$, we get $4 f(S') \geq g(O)$. Also, $f(S \cup F_{\p_{q-1}}) \geq f(S')$ by monotonicity of $f$, together with the previous inequality contradicts the assumption that the claim of the lemma is not true.
\end{proof}

The following lemma follows directly from Lemma~\ref{lem:submodular-one} for $q=k$. 

\begin{lemma}\label{lem:submodular-one-algo}
 The above algorithm outputs for any $\eps>0$ in time $n^{O(1/\eps)}\bc_{\max}\p_{\max}$ a $0.25$-approximate solution with covering value at least $\bc$ and with packing value at most $(1+\eps)\p$.
\end{lemma}
\begin{proof}
 As shown in Lemma~\ref{lem:submodular-one}, the solution output by the algorithm is $0.25$-approximate and has covering value at least $\bc$. If $\p'$ is the weight of the table entry, then the total weight of the solution output is $\p'+\bP \one_{F_{\p'}}\leq \p'+(1+\eps)\p-\p'=(1+\eps)\p$ as claimed.

Observe that the table has $O(n^2\bc_{\max}\p_{\max})$ entries (Line~(\ref{algline:init}, Algorithm~\ref{alg:GreedyDPForbid}) and computing each of the entries takes $O(n)$ time (Line~(\ref{algline:forEachElement}, Algorithm~\ref{alg:GreedyDPForbid}), hence we get the stated running time.
\end{proof}


Using standard scaling techniques, we can bring the running time down to polynomial at the expense of also violating the covering constraint by a factor $(1-\eps)$. 

\begin{lemma}
\label{lem:submodular-one-0.25}
There is an algorithm for maximizing a monotone submodular function subject to one covering and one packing constraint that outputs for any $\eps>0$ in $n^{O(1/\eps)}$ time a $0.25$-approximate solution with covering value at least $(1-\eps)\bc$ and with packing value at most $(1+\eps)\p$.
\end{lemma}
\begin{proof}
We will scale our instance and then apply Lemma~\ref{lem:submodular-one-algo}. First, we can assume that $\bc_{\max} \leq \bc$ because for all elements $\ell$ with covering value strictly larger than $\bc$ we can set $\bC_\ell=\bc$ thereby obtaining an equivalent instance with this property. Similarly, we can assume that $\p_{\max}\leq \p$ by removing all elements $\ell$ with $\bP_\ell>\p$ from the instance.

Let us assume that $\eps\leq 1$. Let $K_\bc=\frac{\eps \bc_{\max}}{n}$ and $K_\p=\frac{\eps \p_{\max}}{2n}$ be ``scaling factors'' and set $\bC_\ell'=\lceil \bC_\ell/K_\bc\rceil$ and $\bP_\ell'=\lfloor \bP_\ell/K_\p\rfloor$ for all $ \ell \in \cN$. Moreover, define new covering and packing bounds $\bc'=\lceil \bc/K_\bc\rceil$ and $\p'=\lfloor \p/K_\p\rfloor$.

Let $O$ be the optimum solution for the original, unscaled covering and packing values. Note that $\bC'\one_O\geq \bc'$ and $\bP'\one_O\leq \p'$ and hence $O$ is a feasible solution also with respect to the instance with scaled scaled covering and packing values $\bC_\ell', \bP_\ell'$ for $\ell\in\cN$ and bounds $\bc',\p'$.

Let $S$ be the solution output by the algorithm of Lemma~\ref{lem:submodular-one-algo} in the down-scaled instance where we use the error parameter $\eps'=\eps/2$. By the claim of the lemma, we have $f(S)\geq 0.25 f(O)$ since $O$ is also feasible in the scaled instance. Moreover, $\bC'\one_S\geq \bc'$ and $\bP'\one_S\leq (1+\eps/2)\p'$.

Now, we prove that the solution $S$ obeys the violation bounds in the \emph{original}, unscaled instance as claimed by the lemma. In fact, for any element $\ell \in\cN$ we have that $K_\bc \cdot \cC_\ell'\leq \bC_\ell+K_\bc$. Hence
\begin{align*}
\bC\one_S & \geq K_\bc\cdot \bC'\one_S - nK_\bc\\
 & = K_\bc\cdot \bC'\one_S - \eps \bc_{\max}\\
 & \geq K_\bc\cdot \bc'-\eps \bc_{\max}\\
 & \geq K_\bc \frac{\bc}{K_\bc}-\eps \bc_{\max}\\
 & \geq (1-\eps)\bc \, .
\end{align*}
Similarly, $K_\p\cdot \bP_\ell'\geq \bP_\ell-K_\p$ and thus
\begin{align*}
\bP\one_S & \leq K_\p\cdot \bP'\one_S +nK_\p\\
 & = K_\p\cdot \bP'\one_S + \frac{\eps}{2} \p_{\max}\\
 & \leq K_\p\cdot \left(1+\frac{\eps}{2}\right)\p'+\frac{\eps}{2} \p_{\max}\\
 & \leq K_\p \left(1+\frac{\eps}{2}\right)\frac{\p}{K_\p}+\frac{\eps}{2} \p_{\max}\\
 & \leq (1+\eps)\p\, .
\end{align*}

By Lemma~\ref{lem:submodular-one-algo} the running time is $n^{O(1/\eps)}\frac{\bc_{\max}}{K_\bc}\frac{\p_{\max}}{K_\p}=n^{O(1/\eps)}$.

\end{proof}


\paragraph{Factor-Revealing LP}
\label{sec:submodular-fact-rev-LP}
Note that in the previous analysis we looked at only \emph{one phase} in which we account for our gain based on whether the element gives us an incremental gain of more than $1/2$ times the incremental gain which it contributes to the optimal solution or not. But in reality for the elements added in the beginning, we gain almost the same value as in the optimal solution and the ratio of gain decreases until we gain $0$ value if we add any element from the optimal which is still not in our solution. In this section we analyze our DP using a factor-revealing LP by discretization of the incremental gain ratios to $1-\frac{1}{m}, 1-\frac{2}{m}, \dots, \frac{1}{m}$ and get lower bounds for the partial solutions at the end of each phase. Then we embed these inequalities into a factor-revealing LP and show that for the worst distribution of the optimal solution among the phases, the approximate solution will be at most a factor $0.353$ away from the optimum solution. 

The $i^{th}$ phase corresponds to the phase in which we will gain at least a $(1-i/m)$-fraction of incremental gain if we add an element from the optimal solution during that iteration. We keep on adding these elements to $O_i$, until no such element remains. $A_i$ corresponds to the solution at the end of the $i^{th}$ phase. $A_m$ is the solution at the end of this procedure. Now we estimate the value of the approximate solution $A_m$ as compared to the optimal solution.

For the purpose of analysis, by scaling, we assume that $f(O) = \sum_{o \in O} g(o)=1$. We set the starting solution $A_0 \triangleq G$ to the set of guessed elements. For the analysis, we also assume that the guessed elements are the first ones in the permutation used to define the function $g$, hence $g(G) = f(G)$.

Now we extend the idea above to forbidden sets. We first do our multi-phase analysis until we reach the solution $A_m = T[p(O\setminus F_m), w(O \setminus F_m)]$, where $F_m$ is the forbidden set corresponding to this table entry. Now we will show that the best of the solutions $A_i \cup F_i$ for $i \in [m]$ has the value at least a factor $0.353$ times the value $g(O) = f(O)$.

The following lemma is the basis of our factor-revealing LP.
\begin{lemma}
\label{lem:submodular-one-multi-phase}
Let $m\geq 1$ be a integral parameter denoting the number of phases. We can pick for each $i \in [m] \cup \{0\}$ a set $O_i = \{o^i_1, o^i_2, \dots o^i_{q_i}\} \subseteq O$ (possibly empty) and an $\alpha_i\in [0,1]$ such that the following holds. For any $i\neq j$, we have that $O_i \cap O_j = \emptyset$. Let $Q_i \triangleq\cup_{j=0}^iO_j$, $\bc_i \triangleq \bC \one_{Q_i}$ and $\p_i \triangleq \bP \one_{Q_i}$ and let $A_i \triangleq T[\bc_i, \p_i]$ be the corresponding entry in the DP table. Then set $O_i$ is disjoint from the forbidden set $F_i \triangleq F_{\p_i}$ for any $i$. Finally, the following inequalities hold:
\begin{enumerate}
\item \label{ineq:o0} $f(A_0) =  g(O_0)$,
\item \label{ineq:o1} $f(A_i) \geq f(A_{i-1}) +  \left(1-\frac{i}{m}\right) g(O_i) \qquad \forall i \in [m]$ and
\item \label{ineq:o2} $f(A_i \cup F_i) \geq f(A_i) + \alpha_i g(F_i \cap O) \qquad \forall i \in \{0\} \cup [m]$.
\item \label{ineq:o3} $f(A_i) \geq \frac{i}{m} \left(1- g(F_i \cap O) - \sum_{j=0}^i g(O_j)\right) + (1 - \alpha_i) g(F_i \cap O) \qquad \forall i \in \{0\} \cup [m]$.
\end{enumerate}
\end{lemma}
\begin{proof}
  We prove this by using induction on $i$. Let $G$ be the set of guessed elements from $O$ in the guessing phase. For $i=0$, inequality \ref{ineq:o0} is trivially true by picking $O_0=A_0=T[\bC \one_G), \bP \one_G] = G$. Let $F_0 = F_{\bP \one_G}$. If $g(F_0 \cap O) = 0$, then the inequalities~\ref{ineq:o2} and~\ref{ineq:o3} are trivially true. Otherwise, let $\alpha_0 = \min\{1, \frac{f(A_0 \cup F_0) - f(A_0)}{g(F_0 \cap O)}$ \}. For this choice inequality~\ref{ineq:o2} holds trivially. Also for $\alpha_0 =1$ the inequality~\ref{ineq:o3} holds trivially. Otherwise $f(A_0) = f(A_0 \cup F_0) - \alpha_0 g(F_0 \cap O) \geq f(F_0 \cap O) - \alpha_0 g(F_0 \cap O) \geq (1-\alpha_0) g(F_0 \cap O)$, which concludes the base case.

For the inductive step let $i \geq 1$ and assume that inequalities \ref{ineq:o1}, \ref{ineq:o2} and \ref{ineq:o3} are true for every $j < i$ (For $i=1$ inequality~\ref{ineq:o0} holds instead of inequality~\ref{ineq:o1}.). We start by defining $O_i \triangleq  \emptyset$, $A_i \triangleq A_{i-1}$ and $F_i = F_{i-1}$. Note that the inequality~\ref{ineq:o1} is true for this choice of $O_i$ and $A_i$. Now if there is an $o \in O \setminus F_i \cup (\cup_{j=0}^{i} O_j)$, such that $f(A_i \cup \{o\}) - f(A_i) > (1-\frac{i}{m}) g(o)$, then this implies that $T[\bC \one_{A_i\cup \{o\}}, \bP \one_{A_i\cup \{o\}}] \geq f(A_i \cup \{o\}) > f(A_i) + (1-\frac{i}{m}) g(o) \geq f(A_{i-1}) + (1-\frac{i}{m})g(O_i) + (1-\frac{i}{m}) g(o) =  f(A_{i-1}) + (1-\frac{i}{m})g(O_i\cup\{o\})$. Note that $o \notin A_i$, since otherwise the left hand side of the inequality will be zero and $g(o)$ is non-negative. Let $Q'_i \triangleq\cup_{j=0}^iO_j \cup \{o\}$. Hence, we can extend $O_i \rightarrow O_i \cup \{o\}$, $A_i \rightarrow  f(T[\bC\one_{Q'_i}, \bP\one_{Q'_i}]$ and $F_i \rightarrow F_{\bP\one_{Q'_i}}$. Hence, inequality \ref{ineq:o1} remains true after performing this operation on $O_i$ and $A_i$. We keep on doing this until for all $o \in O \setminus (F_i \cup (\cup_{j=0}^{i} O_j))$,  $f(A_i \cup \{o\}) - f(A_i) \leq (1-\frac{i}{m}) g(o)$. Then the construction of the set $O_i$ is completed.

Now we show that inequalities~\ref{ineq:o2} and~\ref{ineq:o3} hold as well. Let us define $\alpha_i \triangleq \min\left\{1, \frac{f(A_i \cup F_i) - f(A_i)}{g(F_i \cap O)}\right\}$ if $g(F_i \cap O) \neq 0$, and $\alpha_i \triangleq 1$ otherwise. This definition directly implies inequality~\ref{ineq:o2}.

Assume first that $\alpha_i < 1$. Let $O \setminus (F_i \cup (\cup_{j=0}^i O_j)) = \{ a_1, a_2, \dots, a_q\}$. By submodularity we have that $f(A_i \cup \{a_1, \dots, a_j\})-f(A_i \cup \{ a_1, \dots, a_{j-1}\})\leq f(A_i \cup \{a_j\})-f(A_i)\leq (1-i/m) g(a_j)$ for each $j=1, \dots, q$. We also have $f(A_i \cup F_i \cup (O \setminus (F_i\cup(\cup_{j=0}^i O_j)))) - f(A_i \cup (O \setminus (F_i\cup (\cup_{j=0}^i O_j)))) \leq f(A_i \cup F_i) - f(A_i) = \alpha_i g(F_i \cap O)$ as $\alpha_i<1$. By adding up the previous inequalities for all $j=1, \dots, q$ and the last inequality, we get that
\begin{align*}
f(A_i \cup F_i \cup (O \setminus \cup_{j=0}^i O_j))-f(A_i) &= \sum_{j=1}^q [f(A_i \cup \{a_1,\dots,a_j\})\\
& \qquad\qquad - f(A_i \cup \{ a_1, \dots, a_{j-1}\})] + \alpha_i g(F_i \cap O)\\
& \leq \left(1-\frac{i}{m}\right)  \sum_{j=1}^q g(a_j) + \alpha_i g(F_i \cap O)\\
& = \left(1-\frac{i}{m}\right) g(O \setminus ((\cup_{j=0}^i O_j) \cup F_i)) + \alpha_i g(F_i \cap O)\,.
\end{align*}
Rearranging, we get
\begin{align*}
f(A_i)    & \geq f(A_i \cup F_i \cup (O \setminus \cup_{j=0}^i O_j)) - \left(1-\frac{i}{m}\right) g(O \setminus (F_i \cup (\cup_{j=0}^i O_j))) - \alpha_i g(F_i \cap O) \\
             & \geq f((F_i \cap O) \cup (O \setminus (\cup_{j=0}^i O_j \cup F_i))) - \left(1-\frac{i}{m}\right) g(O \setminus (F_i \cup (\cup_{j=0}^i O_j))) - \alpha_i g(F_i \cap O)\\
             & \stackrel{\text{Lem.~\ref{lem:subset}}}{\geq} \frac{i}{m} g(O \setminus (F_i \cup (\cup_{j=0}^i O_j))) + (1- \alpha_i) g(F_i \cap O) \\
             & = \frac{i}{m} \left(1 - g(F_i \cap O) - \sum_{j=0}^i g(O_j)\right) + (1- \alpha_i) g(F_i \cap O)\,.
\end{align*}

The case $\alpha_i = 1$ is similar to the above and in fact simpler. For the sake of completeness, we state it here. Let $O \setminus (F_i\cup(\cup_{j=0}^i O_j)) = \{ a_1, a_2, \dots, a_q\}$. By submodularity we have that $f(A_i \cup \{a_1, \dots, a_j\})-f(A_i \cup \{ a_1, \dots, a_{j-1}\})\leq f(A_i \cup \{a_j\})-f(A_i)\leq (1-i/m) g(a_j)$ for each $j=1, \dots, q$. Adding up these inequalities for all $j=1, \dots, q$ we get that
\begin{align*}
f(A_i \cup (O \setminus (F_i\cup (\cup_{j=0}^i O_j))))-f(A_i) &= \sum_{j=1}^q [f(A_i \cup \{a_1,\dots,a_j\})\\
& \qquad\qquad - f(A_i \cup \{ a_1, \dots, a_{j-1}\})]\\
& \leq \left(1-\frac{i}{n}\right)  \sum_{j=1}^q g(a_j)\\
                                                            & = \left(1-\frac{i}{m}\right) g(O \setminus (F_i\cup(\cup_{j=0}^i O_j)))\,.
\end{align*}
Rearranging, we get
\begin{align*}
  f(A_i) & \geq f(A_i \cup (O \setminus (F_i\cup(\cup_{j=0}^i O_j)))) - \left(1-\frac{i}{m}\right) g(O \setminus (F_i\cup (\cup_{j=0}^i O_j)))\\
             & \geq f(O \setminus (F_i\cup(\cup_{j=0}^i O_j))) - \left(1-\frac{i}{m}\right) g(O \setminus (F_i\cup(\cup_{j=0}^i O_j)))\\
             & \stackrel{\text{Lem.~\ref{lem:subset}}}{\geq} \frac{i}{m} g(O \setminus (F_i\cup(\cup_{j=0}^i O_j))) \\
             & = \frac{i}{m} \left(1 - g(F_i\cap O)- \sum_{j=0}^i g(O_j)\right)\,.
\end{align*}
This implies that inequality \ref{ineq:o3} is also true for this $A_i$ and $O_i$ and hence the induction follows.


Hence inequality \ref{ineq:o3} is also true and hence the induction follows.
\end{proof}
Below, we state our \emph{factor-revealing} LP that captures the above-described multi-phase analysis with forbidden sets. The idea is to introduce variables for the quantities in the inequalities in the previous lemma and determining the minimum ratio that can be guaranteed by these inequalities.
\begin{align}
\min \,\, & \textstyle c 							      	   								&& \mbox{s.t.} &&  \hspace{11em}  \mbox{(LP-F)} \nonumber \\
	   & \textstyle a_0 = o_0;						     	   								&& \\
           & \textstyle a_i \geq a_{i-1} +  \left(1-\frac{i}{m}\right) o_i                   								&& \forall i \in [m];~\label{lp1:c1} \\ 
           & \textstyle b_i \geq a_i +  g_i			             										&& \forall i \in [m] \cup \{0\};~\label{lp1:c2} \\ 
           & \textstyle a_i \geq \frac{i}{m} (1- f_i - \sum_{j \leq i} o_j)  + f_i - g_i 						&& \forall i \in [m] \cup \{0\};~\label{lp1:c3} \\
           & \textstyle b_i \geq f_i				             										&& \forall i \in [m] \cup \{0\};~\label{lp1:c4} \\ 
           & \textstyle f_i \leq  f_{i-1}		          	      			      							&& \forall i \in [m];\\
           & \textstyle g_i \leq  f_i			          	      			      							&& \forall i \in [m] \cup \{0\};\\
           & \textstyle f_j + \sum_{i=0}^j o_i \leq 1;           	      			      						&& \forall j \in [m] \cup \{0\};\\ 
           & \textstyle c \geq b_i           	      			      										&& \forall i \in [m] \cup \{0\};~\label{lp1:c0} \\ 
           & \textstyle a_i \geq 0, \,\, o_i \geq 0 \,\, f_i \geq 0 \,\, g_i \geq 0	     						&& \forall i \in [m] \cup \{0\}.
\end{align}

The variable $o_i$ corresponds to the incremental gain $g(O_i)$ for the set $O_i$ in our analysis. Variables $a_i$, $b_i$ and $f_i$ correspond to the quantities $f(A_i)$, $f(A_i \cup F_i)$ and $g(F_i)$ for the approximate solution $A_i$ and the corresponding forbidden set $F_i$ for each phase $i=1, 2, \dots, m$. The variable $g_i$ corresponds to the value $\alpha_i g(F_i \cap O)$. We add all the inequalities we proved in Lemma~\ref{lem:submodular-one-multi-phase} as the constraints for this LP (and additional obvious inequalities). Note that since $f(O)=1$, the minimum possible value of $\max_i b_i$ will correspond to a lower bound on the approximation ratio of our algorithm, which is captured by variable $c$ in the LP above.


\paragraph{Upper and Lower Bounds for the Factor-Revealing LP}
\label{subsec:lp_bounds}
For every positive integer $m$, the above factor-revealing LP provides a lower bound on the approximation ratio of our greedy DP described in Section~\ref{subsec:submodular-one}. Ideally, we would like to analytically determine the limit to which this bound converges when $m$ tends to infinity. Unfortunately, giving such a bound seems quite intricate due to the complexity of the LP.

Therefore, we shall first analyze the LP for the case that $f_i=0$ for
all $i\in\{0\}\cup[m]$. This corresponds to the assumption that the
forbidden sets do not contain elements from the optimum
solution. Under this assumption, we are able to analytically determine
the behavior of this simplified LP and show that it converges to
$1/\mathrm{e}$. We shall see that by dropping this assumption we loose a
positive but rather small amount in the approximation ratio.

First consider the following substantially simplified LP.
\begin{align}
\min \,\, & \textstyle a_m 							      && \mbox{s.t.} &&  \hspace{16em}  \mbox{(LP)} \nonumber \\
           & \textstyle a_1 \geq \left(1-\frac{1}{m}\right) o_1;           	      &&~\label{lp:c0} \\ 
           & \textstyle a_i \geq a_{i-1} +  \left(1-\frac{i}{m}\right) o_i            && \forall i \in [m] \setminus \{1\};~\label{lp:c1} \\ 
           & \textstyle  a_i \geq \frac{i}{m} \left(1- \sum_{j \leq i} o_j\right)   && \forall i \in [m];~\label{lp:c2} \\
           & \textstyle a_i \geq 0, \,\, o_i \geq 0 			     && \forall i \in [m].
\end{align}


The following is the dual for the above LP.
\begin{align}
\max \,\,             & \textstyle \sum_{i = 1}^{m} \frac{i}{m} y_i                                    && \mbox{s.t.} && \hspace{13em} \mbox{(DUAL)}  \nonumber \\
		       & \textstyle x_i + y_i - x_{i+1} \leq 0                                               && \forall i \in [m-1];~\label{du:ai} \\
                        & \textstyle x_m + y_m \leq 1; 				   		         &&~\label{du:an} \\
                        & \textstyle \sum_{j \geq i} \frac{j}{m}y_j - (1-\frac{i}{m}) x_i \leq 0	 && \forall i \in [m];~\label{du:oi} \\
                        & \textstyle x_i \geq 0, \,\, y_i \geq 0 			    			 && \forall i \in [m].
\end{align}

We want to show that the optimal value of the LP is at least $\left(1 - \frac{1}{m}\right)^m$. To this end, we will show a feasible dual solution with the same value.  In particular, we let $x_i = \left(1-\frac{1}{m}\right)^{m-i}$ for $i \in [m]$, $y_i = \frac{1}{m}\left(1-\frac{1}{m}\right)^{m-i-1}$ for $i \in [m-1]$ and $y_m = 0$ and show the following lemma. 

\begin{lemma}
\label{lem:submodular-const-dual}
The above solution is a feasible solution for (DUAL). Moreover, the value of this solution is $(1-1/m)^m$.
\end{lemma}
\begin{proof}
The constraint $x_m + y_m \leq 1$ is trivially satisfied since $x_m=1$ and $y_m=0$.

Now let us consider a constraint of the form $x_i + y_i - x_{i+1} \leq 0$. For these constraints the left hand side is equal to
\[
\left(1-\frac{1}{m}\right)^{m-i} + \frac{1}{m}\left(1-\frac{1}{m}\right)^{m-i-1} - \left(1-\frac{1}{m}\right)^{m-i-1}  = \left(1-\frac{1}{m}\right)^{m-i} - \left(1-\frac{1}{m}\right)^{m-i-1}\left(1 - \frac{1}{m}\right) = 0
\]
hence they are satisfied.

For the second kind of constraints $\sum_{j \geq i} \frac{j}{m}y_j - \left(1-\frac{i}{m}\right) x_i \leq 0$, the left hand side is equal to
\[
\sum_{j = i}^{m-1} \frac{j}{m} \frac{1}{m}\left(1-\frac{1}{m}\right)^{m-j-1} - \left(1-\frac{i}{m}\right) \left(1-\frac{1}{m}\right)^{m-i}
\]
First, we simplify the first term 
$T \triangleq \sum_{j=i}^{m-1} \frac{j}{m} \frac{1}{m}(1-\frac{1}{m})^{m-j-1} = \frac{1}{m^2}\sum_{j = i}^{m-1} j \left(1-\frac{1}{m}\right)^{m-j-1}$, 
which is an arithmetic-geometric progression. Now we multiply both sides by $(1-1/m)$ to get, 
$(1-\frac{1}{m})T = \frac{1}{m^2}\sum_{j = i}^{m-1} j (1-\frac{1}{m})^{m-j}$. Subtracting the second equality from first we get,
\begin{align*}
\frac{T}{m} &= \frac{1}{m^2} \left( (m-1) -  \sum_{j=1}^{m-i-1} \left(1-\frac{1}{m}\right)^j - i \left(1-\frac{1}{m}\right)^{m-i} \right) \\
			&= \frac{1}{m^2} \left( (m-1) - \left(1-\frac{1}{m}\right) \frac{1 - \left(1-\frac{1}{m}\right)^{m-i-1}}{\frac{1}{m}} - i \left(1-\frac{1}{m}\right)^{m-i} \right) \\
            &= \frac{1}{m^2} \left( (m-1) - m \left(1-\frac{1}{m}\right) + m \left(1-\frac{1}{m}\right)^{m-i} - i \left(1-\frac{1}{m}\right)^{m-i} \right) \\
            &= \frac{1}{m} \left( \left(1-\frac{1}{m}\right)^{m-i} - \frac{i}{m} \left(1-\frac{1}{m}\right)^{m-i} \right) \\
            &= \frac{1}{m} \left( \left(1-\frac{i}{m}\right)\left(1-\frac{1}{m}\right)^{m-i} \right)
\end{align*}
Which implies that the left hand side of these constraints becomes $0$ and hence they are satisfied. All the $x_i$'s and $y_i$'s are trivially non-negative, which proves the feasibility.

Now we will show that the objective value for this solution is $(1-\frac{1}{m})^m$. Let objective function value corresponding to this solution be $S$. Hence, 
\[
S = \sum_{i = 1}^{m} \frac{i}{m} y_i = y_m +\sum_{i = 1}^{m-1} \frac{i}{m} \frac{1}{m}\left(1-\frac{1}{m}\right)^{m-i-1} = \frac{1}{m^2}\sum_{i = 1}^{m-1} i \left(1-\frac{1}{m}\right)^{m-i-1}
\] 

This is an arithmetic-geometric progression. Hence we multiply both sides by $\left(1-\frac{1}{m}\right)$ to get,
\[
\left(1-\frac{1}{m}\right)S = \left(1-\frac{1}{m}\right) \frac{1}{m^2}\sum_{i = 1}^{m-1} i \left(1-\frac{1}{m}\right)^{m-i-1} = \frac{1}{m^2}\sum_{i = 1}^{m-1} i \left(1-\frac{1}{m}\right)^{m-i}
\]

Subtracting the second equality from first we get,
\begin{align*}
\frac{S}{m} &=  -\frac{1}{m^2} \left(1-\frac{1}{m}\right)^{m-1} + \frac{m-1}{m^2} - \frac{1}{m^2} \sum_{i = 2}^{m-1} \left(1-\frac{1}{m}\right)^{m-i} \\
            &= \frac{1}{m} \left( -\frac{1}{m} \left(1-\frac{1}{m}\right)^{m-1} +\left(1-\frac{1}{m}\right) - \frac{1}{m}\left(1-\frac{1}{m}\right)  \sum_{i = 0}^{m-3} \left(1-\frac{1}{m}\right)^{i} \right) \\
            &= \frac{1}{m} \left( -\frac{1}{m} \left(1-\frac{1}{n}\right)^{m-1} +\left(1-\frac{1}{m}\right) - \frac{1}{m} \left(1-\frac{1}{m}\right) \frac{1-\left(1-\frac{1}{m}\right)^{m-2}}{1/m} \right) \\
            & = \frac{1}{n} \left( -\frac{1}{m} \left(1-\frac{1}{m}\right)^{m-1} + \left(1-\frac{1}{m}\right)  - \left(1-\frac{1}{m}\right) + \left(1-\frac{1}{m}\right)^{m-1} \right) \\
            &= \frac{1}{m} \left(1-\frac{1}{m}\right)^m
\end{align*}
Hence $S=\left(1-\frac{1}{m}\right)^m$, which proves the lemma.
\end{proof}

Now we show that there is a primal feasible solution with matching value to show that the solution is indeed optimal. Let $a_i = \frac{i}{m}\left(1-\frac{1}{m}\right)^{i}$ for $i \in [m]$, $o_i = \frac{1}{m}\left(1-\frac{1}{m}\right)^{i-1}$ for $i \in [m-1]$ and $o_m = 1- \sum_{i=1}^{m-1} o_i$. 

\begin{lemma}
\label{lem:submodular-const-lp}
The above solution is a feasible solution the factor-revealing LP. Moreover, the value of this solution is $\left(1-\frac{1}{m}\right)^m$.
\end{lemma}
\begin{proof}
Note that $a_1 = \frac{1}{m}\left(1-\frac{1}{m}\right) = \left(1-\frac{1}{m}\right) o_1$. Now for any inequality of the type $a_i \geq a_{i-1} +  \left(1-\frac{i}{m}\right) o_i$, the left-hand side is $\frac{i}{n}\left(1-\frac{1}{m}\right)^{i}$. The right-hand side equals 
\[ \frac{i-1}{m}\left(1-\frac{1}{m}\right)^{i-1} +  \left(1-\frac{i}{m}\right) \frac{1}{m}\left(1-\frac{1}{m}\right)^{i-1}  = \left(1-\frac{1}{m}\right)^{i-1} \left(\frac{i}{m} - \frac{1}{m} + \frac{1}{m} - \frac{i}{m^2} \right) = \frac{i}{m}  \left(1-\frac{1}{m}\right)^{i} \]
hence they are satisfied.

Now for any inequality of the type $a_i \geq \frac{i}{m} (1- \sum_{j \leq i} o_j)$ for $i \in [m-1]$, the left-hand side is $\frac{i}{m}(1-\frac{1}{m})^{i}$. The right-hand side equals 
\[\frac{i}{m} \left(1- \sum_{j =1}^i \frac{1}{m}(1-\frac{1}{m})^{j-1} \right) = \frac{i}{m} \left(1- \frac{1}{m}\frac{1 - (1-\frac{1}{m})^i}{1/m} \right) =  \frac{i}{m} \left(1- 1 + (1-\frac{1}{m})^i \right) = \frac{i}{m}(1-\frac{1}{m})^{i} \]

Hence they are satisfied as well. Inequality $a_m \geq  (1- \sum_{j = 1}^m o_j)$ is trivially true by definition of $o_n$. All the $a_i$'s and $o_i$'s (except $o_m$) are trivially non-negative. Finally, $o_m= 1 - \sum_{j = 1}^{m-1} o_j = 1 - \sum_{j =1}^{m-1} \frac{1}{m}\left(1-\frac{1}{m}\right)^{j-1} = 1 - \frac{1}{m}\frac{1 - \left(1-\frac{1}{m}\right)^{m-1}}{1/m} = 1 - 1 + \left(1-\frac{1}{m}\right)^{m-1} \geq 0$, which proves the feasibility for the solution. The objective value for the LP is $a_m=\left(1-\frac{1}{m}\right)^m$, hence the lemma follows.
\end{proof}

From the above to lemmas it follows that the the bounded provided by (LP) converges to $1/\mathrm{e}$ for $m\rightarrow\infty$, which is the approximation ratio of the greedy DP under the above simplifying assumption.

This raises the question if the optimum solution of (LP-F) tends to $1/\e$ for increasing $m$ as well.  Below we show that the bound provided by (LP-F) actually remains below $1/\e-\eps_0$ for any $m$ and for some constant $\eps_0>0$.

Fix an arbitrary positive integer $m$. To show the above claim, we start with the solution $a,o$ described above, which is optimum for (LP). The solution used there is $a_0=0$, $a_i = \frac{i}{m}(1-\frac{1}{m})^{i}$ for $i \in [m]$, $o_i = \frac{1}{m}(1-\frac{1}{m})^{i-1}$ for $i \in [m-1]$ and $o_m = 1- \sum_{i=1}^{m-1} o_i$. Note that by setting $f=g=0$ and $b=a$, we obtain a feasible solution for (LP-F) as well with the same objective function value tending to $1/\e$ for $m\rightarrow\infty$. We now alter this solution so that $f$ attains positive values. This will give us some leverage to alter $o$ and $a$ suitably to actually decrease the objective value by some small positive amount.

We fix parameters $\alpha=0.625, \beta=0.0517, \gamma=0.0647$ More specifically, we set $f_i'=g_i'=\gamma$, $o_i'=o_i-\beta/m$ for $i=1,\dots,m/2-1$.  For $i=m/2$, we set $f_i'=g_i'=0$, $o_i'=o_i+\alpha\beta$. For $i=m/2+1,\dots,m$ we set $f_i'=g_i'=0$ and $o_i'=o_i$. As we specified the values for $o',f'$ and $g'$ the optimum values for $a'$ and $b'$ are ``determined'' in a straightforward way by the inequalities of (LP-F). We give the explicit values below.

The intuition why the above alteration of the solution decreases the objective function value is as follows. We slightly decrease the values of $o_i$ for $i<m/2$. This decreases the RHS of inequality~(\ref{lp1:c1}). We have to compensate for this decrease in two ways. First, by picking $f_i=g_i$ large enough, we ensure that also the RHS of (\ref{lp1:c3}) decreases. We set, however, $f_i=g_i=0$ for $i\geq m/2$ in order to avoid that RHS of~(\ref{lp:c2}) comes too close to $1/\e$ with increasing $i$. To ensure that RHS of~(\ref{lp1:c3}) still decreases, we increase $o_{m/2}$ by \emph{strictly more} ($\alpha>1/2$) than the total decrease of the $o_i$ for $i<m/2$. By picking $\alpha$ not too large, on the other hand, there remains a decrease of the RHS of~(\ref{lp1:c1}) as in this inequality the coefficient of the $o_{m/2}$ is smaller than the coefficients of $o_i$ for $i<m/2$.

\begin{lemma}
\label{lem:upperBoundLPF}
For every $m > 2$, there is a feasible solution $a', b', o', f', g'$ for (LP-F), such that the corresponding objective value for the solution is $1/\e-\beta(\alpha-1/2)/2 + 3\beta/(4m) < 0.3647$.
\end{lemma}
\begin{proof}
We now describe how we pick $a'$ and $b'$. In particular, we set $a_i'=a_i-\beta/ m\sum_{j=1}^i(1-j/m)$, as determined by~(\ref{lp1:c1}), and $b_i'=a_i'+\gamma$ for $i<m/2$. Note that the bound for $a'_{m/2-1}$ by ~(\ref{lp1:c3}) is $a_{m/2-1} - (1/2-1/m)(\gamma - \beta/m(m/2-1))  <   a_{m/2-1} - 0.01942 + 0.0517/m^2 + 0.013/m$ which is smaller than the bound from ~(\ref{lp1:c1}), i.e. $a_{m/2-1} -\beta/ m\sum_{j=1}^{m/2-1}(1-j/m) = a_{m/2-1} - 3\beta/8 + 3\beta/4m >  a_{m/2-1} -0.01939 + 0.038775/m$, for $m\geq 2$. 

For $i=m/2$, we set $a_{m/2}'=a_{m/2}-\beta(\alpha-1/2)/2+3\beta/(4m)$, determined by~(\ref{lp1:c1}). The bound by ~(\ref{lp1:c3}) is $a_{m/2}-\beta(3/4-\alpha)/2- \beta/(2m)$ which is smaller that the previous bound. This, in turn, determines $b_{m/2}'=a_{m/2}'$.  

Finally, we can set $a_i'=a_i-\beta(\alpha-1/2)/2 + 3\beta/(4m)$ and $b_i'=a_i'$ for $i>m/2$ as $o_i'=o_i$ for these values of $i$. These settings yield a feasible solution to (LP-F). The two potential candidates which can determine the objective value are $b'_{m/2-1}$ and $b'_m$. Out of these $b'_m$ is the larger one, which gives an objective value of $1/\e-\beta(\alpha-1/2)/2 + 3\beta/(4m) < 0.3647$, for every $m > 2$.
\end{proof}

Unfortunately, we are not able to analytically determine the approximation ratio to which (LP-F) converges. By computational experiments, we can however show that the answer is not too far from the above upper bound. The following table and the plot shows these bounds for some specific values of $m$ obtained by solving the LP to optimality by means of an LP solver. 

\begin{table}[ht]
\begin{minipage}[b]{0.4\linewidth}
\centering
 \begin{tabular}{ | c | c | }
    \hline
    $m$ & $\min c$ \\
    \hline
    	  2 & 0.25 \\
    	  5 & 0.31727598 \\
        10 & 0.33592079 \\
        50 & 0.34990649 \\
      100 & 0.35160444 \\ 
      500 & 0.35295534 \\ 
    1000 & 0.35312374 \\ 
    2000 & 0.35320790 \\
    5000 & 0.35325839 \\
    \hline
  \end{tabular}
  \caption{Solutions to the (LP-F)}
    \label{tab:opt_lpf}
\end{minipage}\hfill
\begin{minipage}[b]{0.6\linewidth}
\centering
    \includegraphics[width=0.8\textwidth]{OPT_LPF.jpg}
    \captionof{figure}{Growth for the OPT (LP-F) solution}
\label{fig:opt_lpf}
\end{minipage}
\end{table}

Since each of the above (LP-F) values is a valid approximation factor for our algorithm, hence the result for one covering and one packing constraint case stated in Theorem~\ref{thm:submodular-one} follows.\sumi{This part needs polishing}

Finally, if the packing constraint is actually a cardinality constraint we can assume that $\eps<1/\p$. Hence, there will be no violation of the cardinality constraint and also guessing can be avoided. These observations leads to the following lemma, which in combination with the scaling argument used in Lemma~\ref{lem:submodular-one-0.25} finishes the proof for Theorem~\ref{thm:submodular-one}.

\begin{lemma}\label{lem:submodular-card-pseudopoly}
For \PCSM where $p=c=1$ and $\bP=\mathbf{1}_n^{\intercal}$, the Algorithm~\ref{alg:GreedyDPForbid} without the guessing step, outputs for any $\eps>0$ in time $O(n^3\bc_{\max})$ a $0.353$-approximate solution with covering value at least $\bc$ and cardinality $k$.
\end{lemma}
